Chain-of-Dictionary Prompting Elicits Translation in Large Language Models

Large language models (LLMs) have shown surprisingly good performance in multilingual neural machine translation (MNMT) even when trained without parallel data. Yet, despite the fact that the amount of training data is gigantic, they still struggle with translating rare words, particularly for low-resource languages. Even worse, it is usually unrealistic to retrieve relevant demonstrations for in-context learning with low-resource languages on LLMs, which restricts the practical use of LLMs for translation -- how should we mitigate this problem? To this end, we present a novel method, CoD, which augments LLMs with prior knowledge with the chains of multilingual dictionaries for a subset of input words to elicit translation abilities for LLMs. Extensive experiments indicate that augmenting ChatGPT with CoD elicits large gains by up to 13x chrF++ points for MNMT (3.08 to 42.63 for English to Serbian written in Cyrillic script) on FLORES-200 full devtest set. We further demonstrate the importance of chaining the multilingual dictionaries, as well as the superiority of CoD to few-shot demonstration for low-resource languages.

==> case_study.tex <==






% \begin{table*}[ht]
% \setlength{\abovecaptionskip}{4pt}
% \centering
% \small
% \begin{tabularx}{\textwidth}{lX}
% \toprule
% \textbf{Source (eng\_Latn)}& There's a tradition to pass the Easter night awake at some exposed point to see the sunrise. \\
% \textbf{Target ()}&\RL{نەریتێک هەیە بۆ تێپەڕاندنی شەوی ئیستەر بە بەئاگاییەوە لە هەندێک خاڵی ئاشکرا بۆ بینینی خۆرهەڵاتن.} \\
% \hline 
% \textbf{Input}& Translate the following text from English into Kikongo: \{source sentence\} \\
% \textbf{w/o COD}&Mbukale wakutambula Scotturb 403 diambulakala kudimala Sintra, ndumitisa kizidi Cabo da Roca.\\
% \textbf{w/o COD, translated back}& The Scotturb 403 was towed to Sintra, the island of Cabo da Roca. \\
% \hline 
% \textbf{Input}& Based on the given dictionary: 

% "travels" means "lelungan" 

% "regularly" means "ajeg"

% Translate the following text from English into Kikongo: \{source sentence\} \\
% \textbf{Bilingual COD}&Scotturb Bus 403 ekokesa lelungan ajeg ko Sintra, mbika na Cabo da Roca.\\
% \textbf{Bilingual COD, translated back}& Scotturb Bus 403 will connect the airport to Sintra, and then to Cabo da Roca. \\
% \hline 
% \textbf{Input}& Based on the given dictionary: 

% "travels" means "lelungan" means "déplacements" means "Reisen" means "viagens"

% "regularly" means "ajeg" means "régulièrement" means "regelmäßig" means "regularmente" 

% Translate the following text from English into Kikongo: \{source sentence\} \\
% \textbf{COD}&Scotturb Bus 403 ezali ekó longà na Sintra, ya ndeke ezalí na Cabo da Roca.\\
% \textbf{COD, translated back}& Scotturb Bus 403 is heading to Sintra, from the island of Cabo da Roca. \\
% \hline 

% \hline 
% % \textbf{Input}&
% % Based on the given dictionary: 

% % "travels" means "lelungan" means "déplacements" means "Reisen" means "viagens"

% % "regularly" means "ajeg" means "régulièrement" means "regelmäßig" means "regularmente"

% % Translate the following text from English into Kikongo: \textcolor{red}{source sentence}\\ 
% %\hline 
% \textbf{Source}& Some patients might have contracted the bug in the hospital, Dr. Moll thinks, and at least two were hospital health workers.\\
% \textbf{Target}&  Bambefo ya nkaka kubakaka mukolobe/virus yina na lopitalo, Dr. Moll ke yindila, mpi na fioti zole vandaka bisadi minganga ya lopitalo. \\
% \hline 
% \textbf{Input}& Translate the following text from English into Kikongo: \{source sentence\} \\
% \textbf{w/o COD}&Bakoko lela bapómbili bánkulti basídi hôpitala, Dokitá Moll wadila, sôkolô wentu babandílánganî bájiji bángó hôpitala.\\
% \textbf{w/o COD, translated back}& The elderly grandmother was taken to the hospital, Dr. Moll cried, and the school started to rush to the hospital. \\
% \hline 
% \textbf{Input}& Based on the given dictionary: 

% "patients" means "pasien"

% "contracted" means "kontrak" 

% "bug" means "cempé" 

% "hospital" means "rumah sakit" 

% "health" means "kaséhatan" 

% "workers" means "wong kang nyambut gawe" 

% Translate the following text from English into Kikongo: \{source sentence\} \\
% \textbf{Bilingual COD}&Bakoki ba biso bayokana kosepela kamba kosemana na yoto na hospitale, Dr. Moll afundisí buka, mkele banakabakayi laba ni bakangu bana besama bakulekeli kosehéka na hospitali.\\
% \textbf{Bilingual COD, translated back}& Our nurses are not willing to stand on the floor of the hospital, Dr. Moll said, as women and children are sick and exhausted in the hospital. \\
% \hline 
% \textbf{Input}& Based on the given dictionary: 

% "patients" means "pasien" means "patients atteints de" means "Patienten" means "pacientes com"

% "contracted" means "kontrak" means "sous contrat" means "vertraglich" means "contraído"

% "bug" means "cempé" means "démangeaisons" means "Schädel" means "inseto"

% "hospital" means "rumah sakit" means "hôpital" means "Krankenhaus" means "Hospital"

% "health" means "kaséhatan" means "santé" means "Gesundheit" means "saúde"

% "workers" means "wong kang nyambut gawe" means "travailleurs" means "Arbeiter" means "trabalhadores"

% Translate the following text from English into Kikongo: \{source sentence\} \\
% \textbf{COD}&Bakómi bakayinda bàngambó bug, Dr. Moll ba sambéla, na makambo malala nawu nyamú nyamú hospital má kúsòlöla.\\
% \textbf{COD, translated back}& The doctors are fighting the bugs, Dr. Moll said, with pride and the hospital's own ignorance. \\
% \bottomrule
% \end{tabularx}
% \caption{Some examples of the generated compositional instructions.}
% \label{tab:example_ins}
% \vspace{-1.5em}
% \end{table*}






